RD-VIO: Robust Visual-Inertial Odometry for Mobile Augmented Reality in Dynamic Environments

It is typically challenging for visual or visual-inertial odometry systems to handle the problems of dynamic scenes and pure rotation. In this work, we design a novel visual-inertial odometry (VIO) system called RD-VIO to handle both of these two problems. Firstly, we propose an IMU-PARSAC algorithm which can robustly detect and match keypoints in a two-stage process. In the first state, landmarks are matched with new keypoints using visual and IMU measurements. We collect statistical information from the matching and then guide the intra-keypoint matching in the second stage. Secondly, to handle the problem of pure rotation, we detect the motion type and adapt the deferred-triangulation technique during the data-association process. We make the pure-rotational frames into the special subframes. When solving the visual-inertial bundle adjustment, they provide additional constraints to the pure-rotational motion. We evaluate the proposed VIO system on public datasets and online comparison. Experiments show the proposed RD-VIO has obvious advantages over other methods in dynamic environments. The source code is available at: \href{https://github.com/openxrlab/xrslam}{{\fontfamily{pcr}\selectfont https://github.com/openxrlab/xrslam}}.

==> sections/4-2-stabilization.tex <==
\subsection{Stabilization Effect}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{error_curves.pdf}
    \caption{Positioning error curves for the first 20 seconds of the sequence \mhIV{} and \mhV{}.}
    \label{fig:position-error-curve}
\end{figure}

The main goal of the subframes is the better handling of low-translation scenarios.
In the EuRoC dataset, all the sequences have a long period of stopping in the beginning.
By running an algorithm and examine the behavior at these stopped cases, we can see if it can handle them well.
To compare the results, we align the result trajectories at the starting point, then minimize their overall RMSEs by registering them with the best global rotation. This is done using the Umeyama algorithm~\cite{umeyama-tpami-1991}.
Then we can compare the poses with the ground-truth and plot the curve of positioning error.
In Figure~\ref{fig:position-error-curve} we compare the error curves of \sfvio{} and \swvio{} on sequence \mhIV{} and \mhV{}.

The error curve for \swvio{} is jittering when the drone is stopped: its position slowly drifts, then suddenly being ``dragged'' back to a batter location, then drifts again.
This drift is the consequence of missing depth observation -- the positions of the landmarks are becoming more and more inaccurate, and the error in IMU integration is accumulating.
Whenever there is a small purturbation in the translation, the keyframe is added into the sliding window. The bundle adjustment will quickly pick up the new depth observation and correct the pose of the new keyframe, resulting in the ``jittering'' result in its error curve.
Sometimes, the lack of proper depth observation causes \swvio{} produces jumping results, as can be seen around 10th to 11th seconds in sequence \mhV{}.
If the stopping continues, \swvio{} will be starved of reliable landmarks eventually.
This happens for sequence \mhIV{}, after 16 seconds, \swvio{} begin drifting away and was unable to recover to proper tracking.

On the other hand, \sfvio{} was able to accommodate the stopping situation.
Combining with the R-frame marks in Figure~\ref{fig:r-frame-plot}, we can tell that the frames during the stopped time are identified as R-frames, hence are handled in the subframe window.
The compression strategy was able to keep the subframe window short while keeping the IMU bias estimation stable.
In both sequences, the algorithm can keep the tracked position ``locked'' to its place.
Therefore, we can see a smooth and flat error curve during these periods.
